Shape My Moves: Text-Driven Shape-Aware Synthesis of Human Motions

We explore how body shapes influence human motion synthesis, an aspect often overlooked in existing text-to-motion generation methods due to the ease of learning a homogenized, canonical body shape. However, this homogenization can distort the natural correlations between different body shapes and their motion dynamics. Our method addresses this gap by generating body-shape-aware human motions from natural language prompts. We utilize a finite scalar quantization-based variational autoencoder (FSQ-VAE) to quantize motion into discrete tokens and then leverage continuous body shape information to de-quantize these tokens back into continuous, detailed motion. Additionally, we harness the capabilities of a pretrained language model to predict both continuous shape parameters and motion tokens, facilitating the synthesis of text-aligned motions and decoding them into shape-aware motions. We evaluate our method quantitatively and qualitatively, and also conduct a comprehensive perceptual study to demonstrate its efficacy in generating shape-aware motions.

==> figures/fig_motivation.tex <==
\begin{figure}[t]
\centering
\includegraphics[trim=0 0cm 0cm 0.2cm, clip,width=\linewidth]
{images/motivation_v2.pdf}
\caption{
\textbf{Motivation.} Previous methods often preprocess motions by mapping them to a canonical human body model. This normalization step can homogenize diverse body types. As illustrated in the figure, two columns show different subjects performing motions both labeled as 'ballet'. These motions perform differently under different body shapes; however, they are mapped to perform assuming the same canonical body.
}
\label{fig:motivation}
\end{figure}


==> figures/fig_mtk_layout.tex <==

\begin{figure*}[t]
\centering
% \vspace{-5mm}

% \mpage{1.0}{\small{Mean of Each Shape Dimension}}\\

\mpage{1.0}{\frame{\includegraphics[width=\linewidth, trim=0 0cm 0cm 0cm, clip]{images/mtk.pdf}}}\\

\caption{\textbf{Layout of the Perceptual Study.} We show the layout with the collapsible menu item ``Instructions'' on the left and the body of the study on the right. The body consists of the text descriptions at the top, the reference body shape (ground truth body shape corresponding to the shape description) and the two animations to compare in the middle, and the Q\&A block at the bottom.
}
\label{fig:mtk}
\end{figure*}




==> figures/fig_shape_statistic.tex <==

\begin{figure*}[t]
\centering
\vspace{-5mm}

\mpage{1.0}{\small{Mean of Each Shape Dimension with Standard Deviation Represented as Error Bars}}\\

\mpage{1.0}{\includegraphics[width=\linewidth, trim=0 0cm 0cm 1.5cm, clip]{images/beta_satistic.pdf}}\\

\caption{\textbf{Shape Data Statistics in HumanML3D.} We show the mean and standard deviations of the shape $\beta$ parameters to indicate the diversity of body shapes available in the base dataset.
}
\label{fig:shape}
\end{figure*}




==> figures/fig_shape_statistic_addition.tex <==
\begin{figure*}[t]
\centering
% \vspace{-5mm}

\mpage{1.0}{\small{Mean of Each Shape Dimension with Standard Deviation Represented as Error Bars}}\\

\mpage{1.0}{\includegraphics[width=\linewidth, trim=0 0cm 0cm 1.5cm, clip]{images/beta_satistic_addition2k.pdf}}\\

\caption{\textbf{Shape Data Statistics in HumanML3D and Additional Synthetic Shape Data.}
 We show the mean and standard deviations of the shape $\beta$ parameters to indicate the overall diversity of body shapes in the augmented dataset.}
\label{fig:shape_add}
\end{figure*}




==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> tables/multimodality.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Multimodality.}}
\resizebox{.5\columnwidth}{!}{
\begin{tabular}{lc}
\toprule
Method & MModality \\
\midrule
T2M-GPT  & $1.428 ^{\pm 0.055}$ \\
MotionGPT & $8.534 ^{\pm 0.232}$ \\
Ours  & $1.894^{\pm 0.114} $\\
\bottomrule
\end{tabular}
}
\label{tab:multi}
\end{table}

==> tables/physics.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Shape-aware motion synthesis comparison} 
We present a table evaluating the Penetrate, Float, Skate ratio, and bone length variance against the current state-of-the-art methods. We compare our results with the baseline retrained with raw motion data. Our method achieves the best or comparable results, particularly excelling in the Penetrate benchmark, which showcases our model's adeptness at handling raw motion. The category \textit{Shape Input Capability} indicates methods that can incorporate both shape and motion descriptions. Conversely, a lack of this category suggests that the text encoder does not accept shape descriptions as input. \textit{Arbitrary Length} denotes results obtained without using ground-truth motion length. We compare with methods that share the same constraints as ours, capable of generating arbitrary motion lengths and accepting shape descriptions as input. $\colorbox[RGB]{255,179,179}{\:}$ and $\colorbox[RGB]{255,217,179}{\:}$ highlight the best and second-best results.
% We compare our results with the baseline original model and one retrained with raw motion data. Baseline methods do not show significant differences between training with different data sets, revealing an inability to effectively learn physical dynamics, even when trained with unnormalized data. In contrast, our model handles unnormalized motion adeptly, achieving the best or second-best performance in most of the metrics.
}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
% Method & Penetrate (cm)$\downarrow$ & Float (cm)$\downarrow$ & Skate (\%) $\downarrow$ & Bone Length Mean of Variances $\downarrow$ \\
\thead{Methods} & \thead{Shape Input \\ Capability} & \thead{Arbitrary \\ Length} &  \thead{Penetrate ($cm$)$~\downarrow$} & \thead{Float ($cm$)$~\downarrow$} & \thead{Skate ($\%$) $~\downarrow$} & \thead{Bone Length \\ Variances$~\downarrow$} \\

% \thead{Method}  & \thead{Shape-Aware} & \thead{Bone Length\\ Diff. (mm)$\downarrow$} & \thead{Jitter\\ Diff. ($m/s^2$) $\downarrow$} \\

% \cmidrule(lr){6-7}
  % &  &  & &  & {Mean of Variances} & {Difference ($cm$)} \\
\midrule
Real         & - &       -          & $0.0 ^{\pm 0.000}$ & $0.0362 ^{\pm 0.000}$ & $ 7.468^{\pm 0.001}$ & $ 0.0^{\pm 0.000}$ \\
\midrule
% \textbf{Shape-normalized motion} & & & & \\
% TM2T   ~\cite{tm2t} & \xmark   &        \cmark   & $ 0.1317^{\pm 0.005}$ & $ 0.2881^{\pm 0.001}$ & $ 9.587^{\pm 0.001}$ & $ 3.485^{\pm 0.020}$ \\

% T2M ~\cite{t2m}  & \xmark   &        \cmark  &  $ 0.2275^{\pm 0.006}$ & $ 0.2651^{\pm 0.001}$ & $ 7.766^{\pm 0.071}$ & $ 1.110^{\pm 0.074}$ \\

% MLD ~\cite{mld}  & \cmark   &        \xmark &  $ 0.5487^{\pm 0.011}$ & $ 0.4050^{\pm 0.001}$ & $ 9.473^{\pm 0.121}$  & $ 1.759^{\pm 0.025}$ \\

% MotionDiffuse  ~\cite{zhang2022motiondiffuse}& \cmark   &        \xmark  & $ 0.2701^{\pm 0.001}$ & $ 0.3215^{\pm 0.001}$ & $ 6.590^{\pm 0.001}$ & $ 0.190^{\pm 0.002}$ \\

% MDM   ~\cite{mdm} & \cmark   &        \xmark   & $ 0.1013^{\pm 0.001}$ & $ 0.9139^{\pm 0.030}$ & $ 8.085^{\pm 0.141}$ & $ 0.823^{\pm 0.006}$ \\
% \midrule

% T2M-GPT ~\cite{t2mgpt} & \cmark   &        \cmark  & $ 0.5646^{\pm 0.010}$ & $ 0.2915^{\pm 0.004}$ & $ 6.913^{\pm 0.053}$ & $ 1.992 ^{\pm 0.008}$  \\

% MotionGPT ~\cite{motiongpt} & \cmark   &        \cmark & $ 0.6003^{\pm 0.010}$ & $ 0.3265^{\pm 0.008}$ & $ 7.401^{\pm 0.015}$  & $ 1.998 ^{\pm 0.013}$ \\
% \bottomrule
% \textbf{Raw motion} & & & & \\
TM2T   ~\cite{tm2t} & \xmark   &        \cmark & $0.1485 ^{\pm 0.001}$ & $\textcolor{black}{0.2456} ^{\pm 0.001}$ & $ 8.554 ^{\pm 0.001}$ & $ 5.339^{\pm 0.032}$ \\
T2M ~\cite{t2m}  & \xmark   &        \cmark  & $\textcolor{black}{0.0939} ^{\pm 0.001}$ & $0.6805 ^{\pm 0.001}$ & $ \textcolor{black}{4.250} ^{\pm 0.060}$ & $ 1.352^{\pm 0.096}$  \\

MLD ~\cite{mld} & \cmark   &        \xmark  & $0.3091 ^{\pm 0.001}$ & $0.6558 ^{\pm 0.011}$ & $ 9.313 ^{\pm 0.153}$ & $ 2.695^{\pm 0.053}$ \\

MotionDiffuse  ~\cite{motiondiffuse}& \cmark   &        \xmark & $0.2401 ^{\pm 0.001}$ & $0.2703 ^{\pm 0.001}$ & $ 7.710 ^{\pm 0.010}$ & $ \textcolor{black}{0.138}^{\pm 0.002}$ \\
MDM   ~\cite{mdm}  & \cmark   &        \xmark  & $ 0.1011^{\pm 0.001}$ & $ 1.7101^{\pm 0.032}$ & $ 8.523^{\pm 0.150}$ & $ 0.666^{\pm 0.010}$ \\
\midrule
T2M-GPT ~\cite{t2mgpt}& \cmark   &        \cmark  & $\cellcolor{tabsecond}0.1789 ^{\pm 0.004}$ & $0.5241 ^{\pm 0.001}$ & $ \cellcolor{tabsecond}6.162 ^{\pm 0.044}$ & $ \cellcolor{tabsecond}1.176 ^{\pm 0.007}$ \\
MotionGPT ~\cite{motiongpt} & \cmark   &        \cmark & $ 0.6986^{\pm 0.017}$ & $ \cellcolor{tabfirst}{0.2245}^{\pm 0.007}$ & $ 7.889^{\pm 0.078}$  & $ 2.271 ^{\pm 0.018}$ \\
% \midrule
\modelname ~(Ours) & \cmark   &        \cmark &       $ \cellcolor{tabfirst} 0.0268^{\pm 0.001}$       &    \cellcolor{tabsecond}$0.2658 ^{\pm 0.008}$      &     $\cellcolor{tabfirst}{6.143} ^{\pm 0.123}$ & $\cellcolor{tabfirst}{0.625} ^{\pm 0.005}$ \\
\bottomrule
\end{tabular}
}

\label{tab:physic}
\end{table*}


==> tables/physics_norm.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
% Method & Penetrate (cm)$\downarrow$ & Float (cm)$\downarrow$ & Skate (\%) $\downarrow$ & Bone Length Mean of Variances $\downarrow$ \\
Methods & {Penetrate ($cm$)$\downarrow$} & {Float ($cm$)$\downarrow$} & {Skate ($\%$) $\downarrow$} & {Jitter ($m/s^3$) $\downarrow$} & \multicolumn{2}{c}{Bone Length$\downarrow$} \\
\cmidrule(lr){6-7}
  &  &  & &  & {Mean of Variances} & {Difference ($cm$)} \\
\midrule
Real                          & $0.0 ^{\pm 0.000}$ & $0.0362 ^{\pm 0.000}$ & $ 7.468^{\pm 0.001}$ & $ 48.866^{\pm 0.000}$ & $ 0.0^{\pm 0.000}$ & $ 0.0^{\pm 0.000}$  \\
\midrule
TM2T   ~\cite{tm2t}   & $ 0.1317^{\pm 0.005}$ & $ 0.2881^{\pm 0.001}$ & $ 9.587^{\pm 0.001}$ & $ 105.261 ^{\pm 0.150}$ & $ 3.485^{\pm 0.020}$ & $ 15.513^{\pm 0.040}$ \\ 

T2M ~\cite{t2m}    &  $ 0.2275^{\pm 0.006}$ & $ 0.2651^{\pm 0.001}$ & $ 7.766^{\pm 0.071}$ & $ 84.654 ^{\pm 0.131}$ & $ 1.110^{\pm 0.074}$ & $ 7.048^{\pm 0.015}$ \\ 

MLD ~\cite{mld}   &  $ 0.5487^{\pm 0.011}$ & $ 0.4050^{\pm 0.001}$ & $ 9.473^{\pm 0.121}$ & $ 22.775 ^{\pm 0.123}$ & $ 1.759^{\pm 0.025}$ & $ 7.993^{\pm 0.040}$ \\ 

MotionDiffuse  ~\cite{zhang2022motiondiffuse}  & $ 0.2701^{\pm 0.001}$ & $ 0.3215^{\pm 0.001}$ & $ 6.590^{\pm 0.001}$ & $ 40.125^{\pm 0.111}$ & $ 0.190^{\pm 0.002}$ & $ 3.475^{\pm 0.022}$ \\ 

MDM   ~\cite{mdm}    & $ 0.1013^{\pm 0.001}$ & $ 0.9139^{\pm 0.030}$ & $ 8.085^{\pm 0.141}$ & $ 36.365^{\pm 0.359}$ & $ 0.823^{\pm 0.006}$ & $ 12.454^{\pm 0.019}$ \\ 

T2M-GPT ~\cite{t2mgpt}  & $ 0.5646^{\pm 0.010}$ & $ 0.2915^{\pm 0.004}$ & $ 6.913^{\pm 0.053}$ & $ 79.073 ^{\pm 0.013}$ & $ 1.992 ^{\pm 0.008}$ & $ 8.018 ^{\pm 0.018}$ \\ 

MotionGPT ~\cite{motiongpt}  & $ 0.6003^{\pm 0.010}$ & $ 0.3265^{\pm 0.008}$ & $ 7.401^{\pm 0.015}$ & $ 81.011^{\pm 0.204}$  & $ 1.998 ^{\pm 0.013}$ & $ 8.141 ^{\pm 0.019}$ \\ 
\midrule
Ours &       $0.0268 ^{\pm 0.001}$       &    $0.2658 ^{\pm 0.008}$      &     $6.143 ^{\pm 0.123}$ &  $66.233 ^{\pm 0.000}$ &  $0.625 ^{\pm 0.000}$ &  $5.142 ^{\pm 0.000}$     \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Shape-aware motion synthesis Comparison} The Penetrate, Float, Skate ratio is computed using a subset of the dataset that excludes motions involving climbing. This subset selection is intended to ensure the accuracy and relevance of the ratio for motions primarily characterized by ground-based dynamics.}
\label{tab:physic_norm}
\end{table*}


==> tables/physics_unnorm.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Physical Plausibility Comparison} $\colorbox[RGB]{255,179,179}{\phantom{a}}$ and $\colorbox[RGB]{255,217,179}{\phantom{a}}$ highlight the \colorbox[RGB]{255,179,179}{best} and \colorbox[RGB]{255,217,179}{second-best} results.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
% Method & Penetrate (cm)$\downarrow$ & Float (cm)$\downarrow$ & Skate (\%) $\downarrow$ & Bone Length Mean of Variances $\downarrow$ \\
\multirow{2.2}{*}{Methods} & \multirow{1.4}{*}{Shape Input} & \multirow{1.4}{*}{Arbitrary} & 
\multirow{1.4}{*}{Penetrate} & \multirow{1.4}{*}{Float} & \multirow{1.4}{*}{Skate } & \multirow{1.4}{*}{Bone Length} \\
& \multirow{1.0}{*}{Capability} & \multirow{1.0}{*}{Length} & {($cm$)$~\downarrow$} & {($cm$)$~\downarrow$} & {($\%$) $~\downarrow$} & {Variances$~\downarrow$} \\
\midrule
Real         & $-$ & $-$                & $0.0 ^{\pm 0.000}$ & $0.0352 ^{\pm 0.000}$ & $ 8.110^{\pm 0.001}$ & $0.0^{\pm 0.000}$\\
SA-VAE (Recon.)          & $-$ & $-$                &  $0.0289^{\pm 0.000}$ & $0.2090^{\pm 0.000}$ & $6.443^{\pm 0.001}$ & $0.623^{\pm 0.000}$ \\
\midrule
TM2T   ~\cite{tm2t} & \xmark   &        \cmark   & $0.1485 ^{\pm 0.001}$ & $0.2456 ^{\pm 0.001}$ & $ 8.554 ^{\pm 0.001}$ &  $ 5.339^{\pm 0.032}$ \\
T2M ~\cite{t2m}   & \xmark   &        \cmark   & $0.0939 ^{\pm 0.001}$ & $0.6805 ^{\pm 0.001}$ & $ 4.250 ^{\pm 0.060}$ &  $ 1.352^{\pm 0.096}$ \\
MLD ~\cite{mld}  & \cmark   &        \xmark   & $0.3091 ^{\pm 0.001}$ & $0.6558 ^{\pm 0.011}$ & $ 9.313 ^{\pm 0.153}$ &  $ 2.695^{\pm 0.053}$ \\

MotionDiffuse  ~\cite{motiondiffuse}  & \cmark   &        \xmark & $0.2401 ^{\pm 0.001}$ & $0.2703 ^{\pm 0.001}$ & $ 7.710 ^{\pm 0.010}$ &  $ 0.138^{\pm 0.002}$ \\
MDM   ~\cite{mdm}   & \cmark   &        \xmark   & $ 0.1011^{\pm 0.001}$ & $ 1.7101^{\pm 0.032}$ & $ 8.523^{\pm 0.150}$  & $ 0.666^{\pm 0.010}$ \\
\midrule
MotionGPT ~\cite{motiongpt}  & \cmark   &        \cmark  & $ 0.6986^{\pm 0.017}$ & $ \cellcolor{tabfirst} 0.2245^{\pm 0.007}$ & $ 7.889^{\pm 0.078}$   & $ 2.271 ^{\pm 0.018}$ \\
T2M-GPT ~\cite{t2mgpt}  & \cmark   &        \cmark  & $ \cellcolor{tabsecond}0.1789 ^{\pm 0.004}$ & $0.5241 ^{\pm 0.001}$ & $ \cellcolor{tabsecond}6.162 ^{\pm 0.044}$  & $ \cellcolor{tabsecond}1.176 ^{\pm 0.007}$ \\
Ours & \cmark   &        \cmark  &       $ \cellcolor{tabfirst}0.0268 ^{\pm 0.001}$       &    $ \cellcolor{tabsecond}0.2658 ^{\pm 0.008}$      &     $ \cellcolor{tabfirst}6.143 ^{\pm 0.123}$ &   $ \cellcolor{tabfirst}0.625 ^{\pm 0.002}$ \\
\bottomrule
\end{tabular}
}
\label{tab:physic_unnorm}
\end{table*}




% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccc}
% \toprule
% % Method & Penetrate (cm)$\downarrow$ & Float (cm)$\downarrow$ & Skate (\%) $\downarrow$ & Bone Length Mean of Variances $\downarrow$ \\
% Methods & {Penetrate ($cm$)$\downarrow$} & {Float ($cm$)$\downarrow$} & {Skate ($\%$) $\downarrow$} & {Jitter ($m/s^3$) $\downarrow$} & \multicolumn{2}{c}{Bone Length$\downarrow$} \\
% \cmidrule(lr){6-7}
%   &  &  & &  & {Mean of Variances} & {Difference ($cm$)} \\
% \midrule
% Real                          & $0.0 ^{\pm 0.000}$ & $0.0352 ^{\pm 0.000}$ & $ 8.110^{\pm 0.001}$ & $ 48.866^{\pm 0.000}$ & $0.0^{\pm 0.000}$ & $ 0.0^{\pm 0.000}$  \\
% \midrule
% TM2T   ~\cite{tm2t}  & $0.1485 ^{\pm 0.001}$ & $0.2456 ^{\pm 0.001}$ & $ 8.554 ^{\pm 0.001}$ & $ 94.030 ^{\pm 0.183}$ & $ 5.339^{\pm 0.032}$ & $ 26.099 ^{\pm 0.039}$ \\
% T2M ~\cite{t2m}    & $0.0939 ^{\pm 0.001}$ & $0.6805 ^{\pm 0.001}$ & $ 4.250 ^{\pm 0.060}$ & $ 89.523 ^{\pm 0.137}$ & $ 1.352^{\pm 0.096}$ & $ 17.499 ^{\pm 0.046}$ \\

% MLD ~\cite{mld}   & $0.3091 ^{\pm 0.001}$ & $0.6558 ^{\pm 0.011}$ & $ 9.313 ^{\pm 0.153}$ & $ 31.782 ^{\pm 0.201}$ & $ 2.695^{\pm 0.053}$ & $ 16.873 ^{\pm 0.073}$ \\

% MotionDiffuse  ~\cite{zhang2022motiondiffuse} & $0.2401 ^{\pm 0.001}$ & $0.2703 ^{\pm 0.001}$ & $ 7.710 ^{\pm 0.010}$ & $ 42.311 ^{\pm 0.231}$ & $ 0.138^{\pm 0.002}$ & $ 3.925 ^{\pm 0.014}$ \\
% MDM   ~\cite{mdm}    & $ 0.1011^{\pm 0.001}$ & $ 1.7101^{\pm 0.032}$ & $ 8.523^{\pm 0.150}$ & $ 35.281^{\pm 0.270}$ & $ 0.666^{\pm 0.010}$ & $ 11.725^{\pm 0.043}$ \\ 
% T2M-GPT ~\cite{t2mgpt}  & $0.1789 ^{\pm 0.004}$ & $0.5241 ^{\pm 0.001}$ & $ 6.162 ^{\pm 0.044}$ & $ 71.218 ^{\pm 0.122}$ & $ 1.176 ^{\pm 0.007}$ & $ 9.037 ^{\pm 0.019}$ \\ 
% MotionGPT ~\cite{motiongpt}  & $ 0.6986^{\pm 0.017}$ & $ 0.2245^{\pm 0.007}$ & $ 7.889^{\pm 0.078}$ & $ 78.446^{\pm 0.231}$  & $ 2.271 ^{\pm 0.018}$ & $ 17.450 ^{\pm 0.023}$ \\ 
% \midrule
% Ours &       $0.0268 ^{\pm 0.001}$       &    $0.2658 ^{\pm 0.008}$      &     $6.143 ^{\pm 0.123}$ &  $66.233 ^{\pm 0.000}$ &  $0.625 ^{\pm 0.000}$ &  $5.142 ^{\pm 0.000}$     \\
% \bottomrule
% \end{tabular}
% }
% \caption{\textbf{Shape-aware motion synthesis Comparison} }
% \label{tab:physic_unnorm}
% \end{table*}


==> tables/supp_template.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Template for Shape Description Data Input.} This table provides a structured format for users to input detailed measurements of human body attributes. It includes fields for height, weight, body type, and specific measurements for chest, waist, hips, arms, and legs, ensuring comprehensive data collection for shape-aware motion synthesis.}
\begin{tcolorbox}[colback=gray!8, colframe=black!90, boxrule=1pt, sharp corners]
\begin{enumerate}[leftmargin=*]
    \item A \textless{}gender\textgreater{} standing \textless{}height\textgreater{} cm tall, with a chest circumference of \textless{}chest\textgreater{} cm, waist circumference of \textless{}waist\textgreater{} cm, and hip circumference of \textless{}hip\textgreater{} cm. The length of the arm is \textless{}arm\textgreater{} cm and leg height is \textless{}leg\textgreater{} cm.
    \item This individual, a \textless{}gender\textgreater{}, has a height of \textless{}height\textgreater{} cm. Their body measurements include a chest of \textless{}chest\textgreater{} cm, a waist of \textless{}waist\textgreater{} cm, and hips measuring \textless{}hip\textgreater{} cm. The arm extends \textless{}arm\textgreater{} cm and the legs are \textless{}leg\textgreater{} cm long.
    \item The \textless{}gender\textgreater{} stands \textless{}height\textgreater{} cm tall. They have a chest circumference of \textless{}chest\textgreater{} cm, a waist of \textless{}waist\textgreater{} cm, and hips that measure \textless{}hip\textgreater{} cm. The arm and leg measurements are \textless{}arm\textgreater{} cm and \textless{}leg\textgreater{} cm, respectively.
    \item Describing the \textless{}gender\textgreater{}: They are \textless{}height\textgreater{} cm in height, with body measurements that include a chest of \textless{}chest\textgreater{} cm, a waist of \textless{}waist\textgreater{} cm, and hips of \textless{}hip\textgreater{} cm. Additionally, their arm measures \textless{}arm\textgreater{} cm, and their leg height is \textless{}leg\textgreater{} cm.
    \item Here is a \textless{}gender\textgreater{} with a height of \textless{}height\textgreater{} cm. Their measurements are as follows: chest \textless{}chest\textgreater{} cm, waist \textless{}waist\textgreater{} cm, and hips \textless{}hip\textgreater{} cm. The lengths of the arm and legs are \textless{}arm\textgreater{} cm and \textless{}leg\textgreater{} cm respectively.
    \item You see a \textless{}gender\textgreater{} whose physical stature includes a height of \textless{}height\textgreater{} cm. Notable measurements are a chest circumference of \textless{}chest\textgreater{} cm, waist circumference of \textless{}waist\textgreater{} cm, and hip circumference of \textless{}hip\textgreater{} cm, with an arm length of \textless{}arm\textgreater{} cm and leg height of \textless{}leg\textgreater{} cm.
    \item A \textless{}gender\textgreater{} with these dimensions: \textless{}height\textgreater{} cm tall, chest \textless{}chest\textgreater{} cm, waist \textless{}waist\textgreater{} cm, hips \textless{}hip\textgreater{} cm, arm \textless{}arm\textgreater{} cm, and leg height \textless{}leg\textgreater{} cm.
    \item Consider a \textless{}gender\textgreater{} who is \textless{}height\textgreater{} cm tall. They have a chest of \textless{}chest\textgreater{} cm, waist of \textless{}waist\textgreater{} cm, and hips of \textless{}hip\textgreater{} cm. Their arm is \textless{}arm\textgreater{} cm long, and their legs measure \textless{}leg\textgreater{} cm in height.
    \item Profile of a \textless{}gender\textgreater{}: Height of \textless{}height\textgreater{} cm, with a chest measurement of \textless{}chest\textgreater{} cm, waist of \textless{}waist\textgreater{} cm, and hips spanning \textless{}hip\textgreater{} cm. The arm and leg heights are \textless{}arm\textgreater{} cm and \textless{}leg\textgreater{} cm, respectively.
    \item A detailed look at a \textless{}gender\textgreater{}: They stand \textless{}height\textgreater{} cm tall, and feature a chest of \textless{}chest\textgreater{} cm, a waist of \textless{}waist\textgreater{} cm, and hips measuring \textless{}hip\textgreater{} cm. Their arm length is \textless{}arm\textgreater{} cm, and the leg height is \textless{}leg\textgreater{} cm.
\end{enumerate}
\end{tcolorbox}
\label{tab:supp_template}
\end{table*}


==> tables/text2motion.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Guo \etal~\cite{t2m} Benchmark Comparison.} $\colorbox[RGB]{255,179,179}{\phantom{a}}$ and $\colorbox[RGB]{255,217,179}{\phantom{a}}$ highlight the \colorbox[RGB]{255,179,179}{best} and \colorbox[RGB]{255,217,179}{second-best} results.
% \textcolor{red}{Red} and \textcolor{blue}{Blue} highlight the best and second-best results.
}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\multirow{2.2}{*}{Methods} & \multirow{1.4}{*}{Shape Input} & \multirow{1.4}{*}{Arbitrary} & \multicolumn{3}{c}{RPrecision$~\uparrow$} & \multirow{2.2}{*}{FID$~\downarrow$} & \multirow{2.2}{*}{MMDist$~\downarrow$} & \multirow{2.2}{*}{Diversity$~\downarrow$} \\
% & \multirow{2.2}{*}{MModality$\uparrow$} \\
\cmidrule(lr){4-6}
& \multirow{1.0}{*}{Capability} & \multirow{1.0}{*}{Length} & {Top1} & {Top2} & {Top3}  && \\
\midrule
Real                &  -   &  -   & $0.469 ^{\pm 0.002}$ & $0.665 ^{\pm 0.002}$ & $0.769 ^{\pm 0.003}$ & $0.001 ^{\pm 0.000}$ & $3.217 ^{\pm 0.007}$ & $0.000^{\pm 0.000}$ \\
%  & ${-}$        \\ %9.137^{\pm 0.091}
SA-VAE (Recon.)          &  -   &    -      & $ 0.454^{\pm 0.003}$ & $0.645 ^{\pm 0.002}$ & $0.749 ^{\pm 0.002}$ & $0.125 ^{\pm 0.001}$ & $3.308 ^{\pm 0.006}$ & $0.101 ^{\pm 0.097}$ \\
%& ${-}$        \\ 
\midrule
% \textbf{Not Shape-Aware} & & & & & & \\
TM2T   ~\cite{tm2t}   & \xmark   &        \cmark             & $0.374 ^{\pm 0.003}$ & $0.559 ^{\pm 0.003} $ & $0.673 ^{\pm 0.002}$ & $1.671 ^{\pm 0.018}$ & $3.843 ^{\pm 0.009}$ & $0.937 ^{\pm 0.091}$ \\ 
%& $ 2.375^{\pm 0.058}$ \\
T2M ~\cite{t2m}       & \xmark    &       \cmark         & $0.408 ^{\pm 0.003}$ & $0.592 ^{\pm 0.003} $ & $0.697 ^{\pm 0.002}$ & $1.230 ^{\pm 0.023}$ & $3.597 ^{\pm 0.007}$ & $0.430 ^{\pm 0.058}$ \\ 
%& $- ^{\pm 0.083}$ \\
% \bottomrule
% \textbf{Shape-Aware} & & & & & & \\
MLD ~\cite{mld}    &       \cmark & \xmark       & $0.383 ^{\pm 0.002}$ & $0.571 ^{\pm 0.003} $ & $0.680 ^{\pm 0.003}$ & $0.882 ^{\pm 0.024}$ & $3.736 ^{\pm 0.008}$ & $\textcolor{black}{0.020} ^{\pm 0.070}$ \\ 
%& $ 2.521 ^{\pm 0.100}$ \\
MotionDiffuse ~\cite{motiondiffuse}   &       \cmark   & \xmark       & $\textcolor{black}{0.426} ^{\pm 0.002}$ & $ \textcolor{black}{0.616} ^{\pm 0.002} $ & $ \textcolor{black}{0.723} ^{\pm 0.003}$ & $0.563 ^{\pm 0.010}$ & $\textcolor{black}{3.392} ^{\pm 0.006}$ & $ 0.320 ^{\pm 0.070}$ \\ 
%& $ 1.041^{\pm 0.031}$ \\
MDM  ~\cite{mdm} &       \cmark & \xmark  & $0.317 ^{\pm 0.006}$ & $0.490 ^{\pm 0.006} $ & $0.599 ^{\pm 0.007}$ & $0.461 ^{\pm 0.045}$ & $4.180 ^{\pm 0.035}$ & $0.320 ^{\pm 0.083}$ \\
%& $ - ^{\pm 0.100}$ \\ %9.137^{\pm 0.091}
\midrule
MotionGPT ~\cite{motiongpt}  &       \cmark   &    \cmark    & $0.128 ^{\pm 0.002}$ & $0.208 ^{\pm 0.002} $ & $0.271^{\pm 0.002}$ & $1.020 ^{\pm 0.034}$ & $7.055 ^{\pm 0.002}$ & $ 0.389^{\pm 0.095}$ \\
%& $ 8.534 ^{\pm 0.232}$ \\ %9.137^{\pm 0.091}
T2M-GPT ~\cite{t2mgpt}      &       \cmark    &     \cmark        & $\cellcolor{tabsecond}{0.394} ^{\pm 0.003}$ & $\cellcolor{tabsecond}{0.576} ^{\pm 0.003} $ & $\cellcolor{tabsecond}{0.683} ^{\pm 0.002}$ & $\cellcolor{tabsecond}{0.269} ^{\pm 0.010}$ & $\cellcolor{tabsecond}{3.710} ^{\pm 0.008}$ & $\cellcolor{tabsecond}{0.190} ^{\pm 0.061}$ \\
%& $ - ^{\pm 0.100}$ \\ %9.137^{\pm 0.091}
% \midrule
\modelname ~(Ours) &       \cmark & \cmark & $\cellcolor{tabfirst}{0.413} ^{\pm 0.008}$ & $\cellcolor{tabfirst}{0.601} ^{\pm 0.005} $ & $\cellcolor{tabfirst}{0.705} ^{\pm 0.005}$ & $\cellcolor{tabfirst}{0.198} ^{\pm 0.015}$ & $\cellcolor{tabfirst}{3.533} ^{\pm 0.016}$ & $\cellcolor{tabfirst}{0.117} ^{\pm 0.131}$ \\
%& $ - ^{\pm 0.100}$ \\ %9.137^{\pm 0.091}
\bottomrule
\end{tabular}
}
\label{tab:text2motion}
\end{table*}

 % $^\ddagger$


==> tables/vae_rebuttal.tex <==
\begin{table}[t]
\centering
% \captionsetup{font=scriptsize}
\caption{\textbf{Additional VAE Comparisons}}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
\toprule
% \thead{Methods}  & \thead{FID$~\downarrow$} & \thead{Bone Length\\ Diff. ($mm$)$~\downarrow$} & \thead{Jitter\\ Diff. ($m/s^2$) $~\downarrow$} \\
Method  & {FID$~\downarrow$} & {Bone Length Diff. ($mm$)$~\downarrow$} & {Jitter Diff. ($m/s^2$) $~\downarrow$} \\
\midrule
MLD ~\cite{mld}  & $0.239$ & $85.26$ & $\mathbf{22.58}$ \\
% SC-VAE (Ours) &             $\cellcolor{tabfirst}{0.125} $ & $ \cellcolor{tabfirst}{45.88} $ & $ \cellcolor{tabfirst}{31.49}$ \\
SA-VAE (Ours) &             $\mathbf{0.125}$ & $\mathbf{45.88}$ & $31.49$ \\
\bottomrule
\end{tabular}
}
\label{tab:vae_rebuttal}
\end{table}

